Recurrent Independent Mechanisms

Learning modular structures which reflect the dynamics of the environment can lead to better generalization and robustness to changes which only affect a few of the underlying causes. We propose Recurrent Independent Mechanisms (RIMs), a new recurrent architecture in which multiple groups of recurrent cells operate with nearly independent transition dynamics, communicate only sparingly through the bottleneck of attention, and are only updated at time steps where they are most relevant. We show that this leads to specialization amongst the RIMs, which in turn allows for dramatically improved generalization on tasks where some factors of variation differ systematically between training and evaluation.

==> oldfig.tex <==

\begin{figure*}[htb!]
\centering
\begin{2picture}[
    scale=1.0,
    black!50, text=black,
    font=\medium,
    %every node/.append style={font=\medium},
    node distance=1mm,
    dnode/.style={
        align=center,
        % The shape:
        font=\small,
        rectangle,minimum size=10mm,rounded corners,
        % The rest
        inner sep=10pt},
    rnode/.style={
        align=center,
        font=\medium,
        % The shape:
        rectangle,
        minimum width=0m,
        minimum height=6mm,
        rounded corners,
        % The rest
        inner sep=1pt,
        thin, draw},
    tuplenode/.style={
        align=center,
        % The shape:
        rectangle,minimum size=2mm,rounded corners,
        % The rest
        inner sep=5pt},
    darrow/.style={
        rounded corners,-latex,shorten <=5pt,shorten >=1pt,line width=2mm},
    mega thick/.style={line width=2pt}
    ]
\matrix[row sep=8.2mm, column sep=3mm] {
    &&
    &&
    &&
    &&
    &&
    &&
    &&
    &&
    \node (h1r) [rnode, minimum width=10mm, top color=red!40, bottom color = red!40] {$h_{t,1}$};
    &&
    \node (h2r) [rnode, minimum width=10mm, top color=blue!10, bottom color = blue!0] {$h_{t,2}$};
    \\
    \node (h1l) [rnode, minimum width=10mm, top color=red!40, bottom color = red!40] {$h_{t,1}$};
    &&
    \node (h2l) [rnode, minimum width=10mm, top color=blue!10, bottom color = blue!0] {$h_{t,2}$};
    &&
    \node (h3l) [rnode, minimum width=10mm, top color=red!40, bottom color = red!40] {$h_{t,3}$};
    &&
    &&
    \node (h2m1) [rnode, minimum width=10mm, top color=blue!10, bottom color = blue!0] {$h_{t,2}$};
    &&
    \node (h2m2) [rnode, minimum width=10mm, top color=blue!10, bottom color = blue!0] {$h_{t+1,2}$};
    &&
    &&
    \node (h2r1) [rnode, minimum width=10mm, top color=red!40, bottom color = red!40] {$h_{t,3}$};
    &&
    &&
    \node (h2r3) [rnode, minimum width=10mm, top color=red!40, bottom color = red!40] {$h_{t+1,3}$};
    \\
    \node (null_l) [rnode, minimum width=10mm, top color=black!20, bottom color = black!20] {$\emptyset$};
    &&
    \node (xt_l) [rnode, minimum width=10mm, top color=black!20, bottom color = black!20] {$x_t$};
    
    &&
    &&
    &&
    &&
    &&
    &&
    
    \node (null_r) [rnode, minimum width=10mm, top color=black!20, bottom color = black!20] {$\emptyset$};
    &&
    \node (xt_r) [rnode, minimum width=10mm, top color=black!20, bottom color = black!20] {$x_t$};
    
    \\
};

\draw[-latex,shorten <=1pt,shorten >=1pt,thick,color=black!20]  (null_l) to node[]{} (h1l);
\draw[-latex,shorten <=1pt,shorten >=1pt,thick,color=black!80]  (null_l) to node[]{} (h2l);
\draw[-latex,shorten <=1pt,shorten >=1pt,thick,color=black!20]  (null_l) to node[]{} (h3l);

\draw[-latex,shorten <=1pt,shorten >=1pt,thick,color=black!80]  (xt_l) to node[]{} (h1l);
\draw[-latex,shorten <=1pt,shorten >=1pt,thick,color=black!20]  (xt_l) to node[]{} (h2l);
\draw[-latex,shorten <=1pt,shorten >=1pt,thick,color=black!80]  (xt_l) to node[]{} (h3l);

\draw[-latex,shorten <=1pt,shorten >=1pt,thick,color=blue!80]  (h2m1) to node[label=above:id]{} (h2m2);
\draw[-latex,shorten <=1pt,shorten >=1pt,thick,color=red!80]  (h2r1) to node[label=above:$D_3$]{} (h2r3);


\draw[-latex,shorten <=1pt,shorten >=1pt,thick,color=red!30]  (h1r) to node[]{} (h2r3);
\draw[-latex,shorten <=1pt,shorten >=1pt,thick,color=blue!30]  (h2r) to node[]{} (h2r3);

\draw[-latex,shorten <=1pt,shorten >=1pt,thick,color=black!20]  (null_r) to node[]{} (h2r1);
\draw[-latex,shorten <=1pt,shorten >=1pt,thick,color=black!80]  (xt_r) to node[]{} (h2r1);




\end{tikzpicture}
\caption{An illustration of the mechanics of the Recurrent Independent Mechanisms (RIMs) model with ($K=3$ RIMs and $k_A=2$ RIMs active at any given point in time; in our applications, we generally use $K>5$ and $k_A=4$).  We use an attention mechanism to select the active RIMs (shown in red) based on the magnitude of their attention weights on the input $x_t$ (left).  This leads the non-activated RIM $\color{blue!70!black} h_{t,2}$ to remain unchanged on that step (middle).  It leads the activated RIMs to be updated using the input attention, then the independent RIM-specific dynamics $\color{red!80!black} D_{3}$, then the communication between RIMs (right, shown for a single activated RIM $\color{red!80!black} h_{t,3}$).  }
\end{figure*}


